Mani-GS: Gaussian Splatting Manipulation with Triangular Mesh

Neural 3D representations such as Neural Radiance Fields (NeRF), excel at producing photo-realistic rendering results but lack the flexibility for manipulation and editing which is crucial for content creation. Previous works have attempted to address this issue by deforming a NeRF in canonical space or manipulating the radiance field based on an explicit mesh. However, manipulating NeRF is not highly controllable and requires a long training and inference time. With the emergence of 3D Gaussian Splatting (3DGS), extremely high-fidelity novel view synthesis can be achieved using an explicit point-based 3D representation with much faster training and rendering speed. However, there is still a lack of effective means to manipulate 3DGS freely while maintaining rendering quality. In this work, we aim to tackle the challenge of achieving manipulable photo-realistic rendering. We propose to utilize a triangular mesh to manipulate 3DGS directly with self-adaptation. This approach reduces the need to design various algorithms for different types of Gaussian manipulation. By utilizing a triangle shape-aware Gaussian binding and adapting method, we can achieve 3DGS manipulation and preserve high-fidelity rendering after manipulation. Our approach is capable of handling large deformations, local manipulations, and soft body simulations while keeping high-quality rendering. Furthermore, we demonstrate that our method is also effective with inaccurate meshes extracted from 3DGS. Experiments conducted demonstrate the effectiveness of our method and its superiority over baseline approaches.

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/itr.tex <==
\section{Introduction}
\label{sec:intro}
% dirty, non, non, high fidelity, same style
Free-view human synthesis or rendering is essential for various applications, including virtual reality, electronic games, and movie production. Traditional approaches often require a dense camera rig or depth sensors to reconstruct the geometry and refine the texture of the subject, resulting in a tedious and time-consuming process.

% Recently, with the advent of the implicit field, remarkable progress has been made in 3D human free-view synthesis from a single RGB image. Some methods \cite{saito2019pifu, saito2020pifuhd, zheng2021pamir}, achieve this by using pixel-aligned 2D image features as input conditions for subsequent occupancy and color prediction of corresponding 3D points. They extract a mesh from the implicit field and predict the vertex color for free-view rendering. However, their rendering results exhibit over-smooth and less fine details due to the lack of novel view information and smoothness bias of implicit field. Some work\cite{huang2023one, gao2022mps, hu2023sherf} build neural radiance field from single image or multi-view images, the rendering results is also

Recently, with the advent of the implicit field, remarkable progress has been made in 3D human free-view synthesis from a single RGB image. Some methods \cite{saito2019pifu, saito2020pifuhd, zheng2021pamir}, achieve this by using pixel-aligned 2D image features as input conditions for subsequent occupancy and color prediction of corresponding 3D points. They extract a mesh from the implicit field and predict the vertex color for free-view rendering.  Some work \cite{huang2023one, gao2022mps, hu2023sherf} build neural radiance fields from single image or multi-view images. However, both rendering results exhibit over-smooth and less fine details due to the lack of novel view information and the smoothness bias of the implicit field. To forecast the invisible information, some methods \cite{qian2023magic123, melas2023realfusion, xu2023neurallift} introduce a 2D text-to-image generative model as guidance and conduct score-distillation-sampling \emph{(SDS)} to optimize a 3D representation for general object. The pipeline also works for human cases, as shown in our concurrent work \cite{huang2023tech}. Nevertheless, \emph{SDS} leads to an over-saturation and over-smooth prediction in the back view which is not texture-consistent with the input reference image, especially with not accurate text prompts. 

In this paper, we aim to achieve texture-consistent human free-view rendering with high fidelity from a single image. However, this problem is extremely challenging. We propose an innovative framework named "ConTex Human". Under this framework, we decompose our ultimate goal into two key sub-targets. The first one is how to generate a texture-consistent back view with fine details. The second one is how to paint the side and invisible region with reasonable texture region after mapping the reference and back view on the reconstructed geometry.

For back view synthesis, we are inspired by recent 2D image/video editing methods \cite{cao2023masactrl, meng2021sdedit, qi2023fatezero, wu2023tune}, which could maintain the style and texture of the original image in editing. Our key idea is to query image contents from the input reference image to generate a texture-consistent human back view through attention injection guided by text prompts. However, naively generating using only text prompts would lead to misalignment between the back view and human geometry. Therefore, we controlled this process with the depth map as guidance to ensure that the generated back view layout is well-aligned with human geometry. After mapping the reference view and back view on the geometry, we need to paint the side region and invisible region. An intuitive solution would be conducting \emph{SDS} on the given person to leverage the 2D Diffusion model prior. But \emph{SDS} only results in color distortion and over-saturation texture. To address this problem, we propose a \emph{visibility-aware patch consistency} loss to alleviate the inconsistent side view texture, which makes sure that the side and invisible region pixel value should be close to its neighbor pixels in the front or back region.

We evaluate our approach on both synthetic dataset THuman2 that has 3D textured scans as ground truth and real dataset SSHQ which includes people in various poses, clothing, and shapes. Across the experiments, our approach exhibits significant performance in both quantitative and qualitative comparisons.

In summary, this work has the following contributions:

\begin{itemize}

    \item We introduce an innovative framework called ``ConTex-Human'', which could achieve high fidelity free-view human rendering with consistent texture from single image.
    % \vspace{pt}    

    \item We design a depth and text prompt conditioned back view synthesis module that could maintain texture style and details in reference images.
    % \vspace{5pt}    
    
    \item To remove the over-saturation texture caused by \emph{SDS}, we proposed a front-back texture mapping module. A \emph{visibility-aware patch consistency} loss is also included to further alleviate the color distortion.


\end{itemize}


% To overcome these problems, in this paper, we propose an innovative framework for texture-consistent human free-view rendering with high fidelity from a single image. We are inspired by recent 2D image/video editing methods \cite{cao2023masactrl, meng2021sdedit, qi2023fatezero, wu2023tune}, which could maintain the style and texture of the original image in editing. Our key idea is to query image contents from the input reference image to generate a texture-consistent human back view through attention injection guided by text prompts and depth map. With generated 






